LeRoP: A Learning-Based Modular Robot Photography Framework

We introduce a novel framework for automatic capturing of human portraits. The framework allows the robot to follow a person to the desired location using a Person Re-identification model. When composing is activated, the robot attempts to adjust its position to form the view that can best match the given template image, and finally takes a photograph. A template image can be predicted dynamically using an off-the-shelf photo evaluation model by the framework, or selected manually from a pre-defined set by the user. The template matching-based view adjustment is driven by a deep reinforcement learning network. Our framework lies on top of the Robot Operating System (ROS). The framework is designed to be modular so that all the models can be flexibly replaced based on needs. We show our framework on a variety of examples. In particular, we tested it in three indoor scenes and used it to take 20 photos of each scene: ten for the pre-defined template, ten for the dynamically generated ones. The average number of adjustment was $11.20$ for pre-defined templates and $12.76$ for dynamically generated ones; the average time spent was $22.11$ and $24.10$ seconds respectively.

==> comments.tex <==
\section{Comments}

1. The potentially most interesting component is the DRL method, but insufficient detail is given to understand it.  More fundamentally, it is unclear why the method is based on learning at all.  The system appears to possess all information and sensors required to determine the vantage point by reasoning about geometry.

2. Although the introduction discusses what properties make a
good shot, such as lighting, framing or composition, there
is little discussion in the paper on how such criteria
should be optimised. The use of templates provide a simple
way to avoid those issues, but it would have been
interesting to try to optimise this important aspect of the
problem. 

3. Although the application is interesting, the
experimental testing of the system is minimal. It would
have been interesting to provide more extensive testing and
analysis of the system's performance in varied conditions.
Also, some evaluation of the system's output (eg, ratings
by users) would have been welcome. Similarly, some
components, such as a the template matching could have been
analysed more rigorously.

4. The description of the tracker module takes too much space for
a subsystem which, if I understand it well, does not
contribute really to the state of the art in person
tracking but reuses other methods. 

5. You describe in fact two different systems for the
tracking (figs. 5b and 5c). I think this does not
contribute to make the paper clearer. It would be much
better if you simply describe the approach that you have
finally chosen (which is, if I am correct, the Yolo one).

6. How do you determine the model of the person to track in
the first place? I think that the problem is not easy as
the quality of the tracking will probably depend a lot on
this first image of the person of interest. 

7. You mention that the candidate person with the highest
similarity is chosen as the target; however, I wonder what
happens when Yolo, for some reason, could not detect the
target. Will you select a badly ranked candidate in that
case? For example, in Fig. 5c, there are 3 detections with
quite high scores (0.78, 0.8, 0.91). If the correct person
is not detected, could this trigger some critical failure
in your system?

8. The vector v 
present in the Equation 1 is not clear at all: Is this the
same as the pose vector which is given as an output from
Openpose? If not, how do you define it and how do you use
the pose vector. Also, what value of alpha did you choose
and why?

9. The third part (final photo acquisition) is not
necessary at all. \hk{I do not think we should remove it.}

10. I would have liked to see a better motivation of the
use of a DRL technique here; intuitively, given the size,
the location, and the desired pose, there should be an
optimal pose of the robot/camera to do the shot; so given
the few degrees of freedom of the robot, a much simpler
scheme may be more efficient.

Another important point that is not answered in the paper
is why the geometric constraints are not used to find the
possible locations of the robot for taking a photo. Since
the human location is known and the pre-defined template is
available, the approximate distance (depth) to the user can
be found by using the RGB-D sensor, which is already used
for tracking. 

11. \sout{The
robot should always be in close proximity to the human,
otherwise the human may move fast and the path to track the
human cannot be found by the robot. A method which is
computationally less expensive (e.g. [1]) can be considered
to compare. 
Z Kalal, K. Mikolajczyk, and J. Matas,
Tracking-Learning-Detection, Pattern Analysis and Machine
Intelligence 2011.}


12. \sout{It is not mentioned if the tracking runs
on the remote computer or on the robot.}

13. It is stated that cosine similarity is used to compare the
ground truth person image with the cropped candidate person
image. Which color space is used for comparison?

14. It is considered that the View Evaluation Net gives the
best candidate template for the dynamical view selection. A
small survey for this assumption for the given conditions
(indoors full body portrait photos) would be helpful to
validate this assumption. Also I could not find the number
of candidate templates generated.

15. A new DRL model is necessary for each
of new pose template. Although this may be feasible for a
small number of pose templates, this would increase the
number of models significantly for pose templates with more
than one person. I think this point needs some discussion
for clarification.

16. The font in Fig.3 can be enlarged.

17. Should there be page numbers? -TJ

==> source/07-acknowledgment.tex <==
\section*{Acknowledgment}

This work was supported by Adobe Research. The authors would like to thank Suren Deepak Rajasekaran for the help on video editing, and Booker Smith for useful discussions. The authors also would like to thank the anonymous reviewers for valuable feedback.

%The work is supported by the \grantsponsor{}{}{} under Grant
%No.:~\grantnum{}{}.



